On d-ary tree algorithms with successive interference cancellation

In this paper, we outline the approach for the derivation of the length of the collision resolution interval for d-ary tree algorithms (TA) with gated access and successive interference cancellation (SIC), conditioned on the number of the contending users. This is the basic performance parameter for TA with gated access. We identify the deficiencies of the analysis performed in the seminal paper on TA with SIC by Yu and Giannakis, showing that their analysis is correct only for binary splitting, i.e. for d=2. We also provide some insightful results on the stable throughput that can be achieved for different values of d.

==> conclusions.tex <==
\section{Discussion and Conclusions}
\label{sec:conclusion}




==> introduction.tex <==
\section{Introduction}
\label{sec:Intro}

In the last decade, there have been significant theoretical advances in the area of random-access protocols, instigated by the novel use-cases pertaining to the Internet of Things (IoT).
A typical IoT scenario involves a massive number of sporadically active users exchanging short messages.
The sporadic user activity mandates the use of random-access protocols, however, their use in massive IoT scenarios faces the challenge of an increased requirement for efficient performance.
Particularly, as the amount of exchanged data is low, the overhead of the random-access scheme should be minimal in order not to create the bottleneck in the overall communication setup.

A way to improve the performance of random-access protocols is to embrace the interference from the contending users. Another well-explored line of research in the context of slotted ALOHA is the use of \ac{SIC} across slots. In this class of protocols~\cite{PSLP2014}, the users transmit multiple replicas of their packets on purpose. Decoding of a packet replica occurring in a singleton slot enables removal of all the other related replicas, potentially transforming some of the collision slots into singletons from which packets of other contending users can be decoded, and thus propelling new iterations of \ac{SIC}, etc.
The use of \ac{SIC} pushes the throughput performance significantly, asymptotically reaching the ultimate bound for the collision channel of 1~\rm{packet/slot}~\cite{L2011,Liva2015:CodedAloha}.


A tree-algorithm based scheme exploiting \ac{SIC}, named SICTA, was proposed by Yu and Giannakis in~\cite{SICTA}.
It was shown that the \ac{MST} of SICTA reaches $\ln 2 \approx 0.693$~packet/slot, which is significantly better than the best performing variant of the algorithm without \ac{SIC}~\cite{V1986}.
The analysis in~\cite{SICTA} considered the general case of $\tf$-ary splitting.
However, in this paper, we show that the underlying model is incorrect for $d > 2$, making the conclusions effective only for the case of binary splitting.

The rest of the text is organized as follows.
In Section~\ref{sec:background} we state the background and briefly review the related work.
Section~\ref{sec:model} formulates the system model.
In Section~\ref{sec:analysis}, we derive the basic performance parameters, which are the expected \ac{CRI} and throughput, conditioned on the number of initially colliding users, followed by the derivation of their asymptotic values as well as upper and lower bounds.
Section~\ref{sec:arrivals} investigates the \ac{MST} performance of the scheme in the case of Poisson arrivals, both for the gated and the windowed access.
Section~\ref{sec:d-ary} considers the general, $\tf$-ary version of the scheme.
Section~\ref{sec:conclusion} concludes the paper.



%In its core, our study is based on the extension of the method elaborated in~\cite{MF1985}
